A survey for variable young stars with small telescopes: II -- Mapping a protoplanetary disk with stable structures at 0.15 AU

The HOYS citizen science project conducts long term, multifilter, high cadence monitoring of large YSO samples with a wide variety of professional and amateur telescopes. We present the analysis of the light curve of V1490Cyg in the Pelican Nebula. We show that colour terms in the diverse photometric data can be calibrated out to achieve a median photometric accuracy of 0.02mag in broadband filters, allowing detailed investigations into a variety of variability amplitudes over timescales from hours to several years. Using GaiaDR2 we estimate the distance to the Pelican Nebula to be 870$^{+70}_{-55}$pc. V1490Cyg is a quasi-periodic dipper with a period of 31.447$\pm$0.011d. The obscuring dust has homogeneous properties, and grains larger than those typical in the ISM. Larger variability on short timescales is observed in U and R$_c-$H$\alpha$, with U-amplitudes reaching 3mag on timescales of hours, indicating the source is accreting. The H$\alpha$ equivalent width and NIR/MIR colours place V1490Cyg between CTTS/WTTS and transition disk objects. The material responsible for the dipping is located in a warped inner disk, about 0.15AU from the star. This mass reservoir can be filled and emptied on time scales shorter than the period at a rate of up to 10$^{-10}$M$_\odot$/yr, consistent with low levels of accretion in other T Tauri stars. Most likely the warp at this separation from the star is induced by a protoplanet in the inner accretion disk. However, we cannot fully rule out the possibility of an AA Tau-like warp, or occultations by the Hill sphere around a forming planet.

==> Analysis.tex <==
\section{Analysis of the data for the light curve of V1490Cyg}
\label{Analysis}

\begin{figure}
\centering
\makebox[\textwidth][c]{\includegraphics[width=0.7\textwidth]{images/U_lightcurve.pdf} \hfill \includegraphics[width=0.7\textwidth]{images/B_lightcurve.pdf} }\\%
\vspace{0.3cm}
\makebox[\textwidth][c]{\includegraphics[width=0.7\textwidth]{images/V_lightcurve.pdf} \hfill \includegraphics[width=0.7\textwidth]{images/R_lightcurve.pdf} }\\%
\vspace{0.3cm}
\makebox[\textwidth][c]{\includegraphics[width=0.7\textwidth]{images/I_lightcurve.pdf} \hfill \includegraphics[width=0.7\textwidth]{images/HA_lightcurve.pdf} }\\%
\caption{Light curves of U, B, V, r, i and \ha\ data for V\,$1490$\,Cyg.}
\label{fig:lightcurves}
\end{figure}

The long-term light curves of V\,$1490$\,Cyg, observed between 2016 and September 2019 in filters U, B, V, r, i and \ha\ are shown in Fig.\,\ref{fig:lightcurves}. The source is also known as $2$MASS\,J$20505357$+$4421008$. It is located at $RA = 20:50:53.58$, $DEC = +44:21:00.9$ (J2000), in the Pelican Nebula, IC\,$5070$.

The recently discovered low-mass YSO is classified as an emission-line object; \citet{2002AJ....123.2597O} having detected \ha\ emission in its spectrum. \citet{2003AstL...29..468S} determined it to be a Variable Star of Orion Type ($Or^*$). It is not listed in \citet{2013ApJ...768...93F} who surveyed the area using data from the Palomar Transient Factory nor is it included in the ASAS-N variable stars database.  V\,$1490$\,Cyg was  however included in the list of candidates for YSOs published by \citet{2009ApJ...697..787G} and has been further studied by \citet{2018RAA....18..137I}, who do not report any periodicity.

Despite this, the object shows strong variability, with large amplitude changes in all filters (U, B, V, r, i and \ha). Table\,\ref{tab:flux_variations} shows the range of variability in each filter giving the maximum amplitude recorded, the minimum amplitude and the amplitude difference ($\Delta$). The brightness variations of V\,$1490$\,Cyg shown are seen over the whole length of observations.

\begin{table}[]
    \caption{Ranges in amplitude for each given filter for V\,$1490$\,Cyg. Given are the minimum recorded magnitudes, the maximum recorded magnitudes and the difference between them.}
    \label{tab:flux_variations}
    \centering
    \begin{tabular}{cccc}
        Filter & min & max & $\Delta$ \\
        \textbf{U} & 18.16 & 14.97 & 3.19 \\
        \textbf{B} & 18.65 & 15.32 & 3.33 \\
        \textbf{V} & 17.27 & 14.83 & 2.44 \\
        \textbf{r} & 15.98 & 13.34 & 2.64 \\
        \textbf{i} & 15.25 & 13.63 & 1.62 \\
        \textbf{\ha} & 16.48 & 10.73 & 5.76 \\
    \end{tabular}
\end{table}

In addition to the large amplitude changes observed, flux variation is present on a range of timescales. Notable in the middle two panels and the bottom left panel in Fig.\,\ref{fig:lightcurves} is the long-term variation. The increased cadence seen between Julian dates ??? and ??? are the result of a focused \hc\ campaign. Participants were encouraged to image the Pelican Nebula as often as they were able, producing a detailed view of the variability on timescales of hours.

All U-band data presented in this thesis is solely taken with the Thuringian State Observatory (see Appx.\,\ref{tls}). Variability also occurs over very short timescales, with amplitudes of up to $2.5$\,mag seen in a matter of hours. The bottom panel in Fig.\,\ref{fig:ds9_plots} displays such short timescale behaviour in the U-band.

This high degree of variability is able to be seen with the naked eye. Figure\,\ref{fig:ds9_plots} shows a 3x3 grid of observations taken in sequence over the course of approximately $7$\,hours. Shown in the panel below is the light curve at this time frame. The highlighted object is V\,$1490$\,Cyg and is seen to dim and brighten according to the variability in the light curve shown in the bottom panel.

\begin{figure}
    \centering
    \includegraphics[width=12cm, height=12cm]{images/ds9.png}
    \caption{\textbf{3x3 grid:} Numbered 1 -- 9 left to right and top to bottom. The highlighted object is V\,$1490$\,Cyg exhibiting dimming and brightening as shown in the light curve below. \textbf{Bottom:} A section of the U-band light curve of V\,$1490$\,Cyg. The data displayed was taken on $9^{\rm th}$ September 2018 (JD $2458371$). It shows the high variability of the star over timescales of hours. The observed variability order is matched with images 1 -- 9 in the 3x3 grid above.}
    \label{fig:ds9_plots}
\end{figure}

The quasi-periodic behaviour of V\,$1490$\,Cyg is observed to have similar timescales for broadband filters B, V, r and i. Visual inspection of these filters' data indicates a periodicity of roughly $31.5$\,days. Such dimming events are not strictly regular however. Short timescale analysis shows that the shape of consecutive dips change. Further, the dimming behaviour is not constant over the entirety of the light curve. For example, several dimming events appear to be missing for a given rough $30$\,day period. One such event occurs around the Julian date of $2458570$.

The occultations seen change duration and depth and last up to $70$\;\% of the estimated period.

%----------------------------------------------------------------------------------------
%	Periodic Dipping Behaviour
%----------------------------------------------------------------------------------------
\subsection{Periodic Dipping Behaviour}
\label{Analysis:Periodic_Dipping_Behaviour}

The \hc\ project has accrued data on the variability of V\,$1490$\,Cyg since 2016. To more accurately determine the periodicity of V\,$1490$\,Cyg, long-term BVRI photometric data of V\,$1490$\,Cyg collected by \citep{2019yCatp040001801I} during the period from September 2010 to October 2017 are presented alongside the \hc\ data. 

All \citep{2019yCatp040001801I} CCD observations of V\,$1490$\,Cyg were obtained with the 50/70-cm Schmidt telescope located at the Rozhen National Astronomical Observatory in Bulgaria. A total of $119$ observational nights were used to estimate the brightness of the object. Observations were performed with the FLI\,PL$16803$ CCD camera. All technical parameters and specifications for the camera used is given in \citet{2015PASA...32...21I}. The images were taken through a standard Johnson-Cousins (BVri) set of filters. Frames were dark subtracted and flat field corrected. The photometric data were reduced using an IDL based DAOPHOT subroutine. A reference of 11 stars reported in \citet{2018PASA...35....7I} was used as a comparison sequence in BVri. All data were analysed using the same aperture, which was chosen to have a $4$\,\arcsec radius, while the background annulus was taken from $9$ to $14$\,\arcsec. The mean value of errors in the reported magnitudes is $0.01-0.02$\,mag for the i- and r-band data and $0.01-0.03$\,mag for the V- and B-band data.

To determine the correct periodicity of V\,$1490$\,Cyg, a Lombscargle periodogram search was run for V, r and i filters. The top left panel of Fig.\,\ref{fig:periodogram_V} shows the V data of V\,$1490$\,Cyg. A period of $31.467000$\,days was found, generated over a timescale of $\approx9$ years. Similar periods are found for r- and i-band data with $31.466944$ and $31.467038$\,days found respectively. The corresponding periodograms are shown in Figs.\,\ref{fig:periodogram_R} and \ref{fig:periodogram_I}. The bottom panels in each of these figures show the phase-folded light curve for each filter, for the obtained period.

Taking the mean of these three calculated periods, a period of $31.46699$\,days is determined  which I will adopt throughout this thesis as the periodicity of V\,$1490$\,Cyg. The standard deviation in periodicity for Vri is $0.0000386$\,days or $3.3$\,seconds.

In comparison, the periodicity of V\,$1490$\,Cyg using only \hc\ data may be calculated in the same manner. A period of $31.484839$\,days was found for V, generated over a timescale of $\approx9$ years. Similar periods are found for r- and i-band data with $31.550053$ and $31.434378$\,days found respectively. Again taking the mean of these three calculated periods, a period of $31.48976$\,days is determined with a standard deviation of $0.0473518$\,days or $4091.19765621582$\,seconds/ $68.186627603597$\,minutes / $1.1364437933932834$\,hours.

The error of $0.0473518$\,days was calculated over an average of $1359.5$\,days in Vri using just the \hc\ data. The data from \citep{2019yCatp040001801I} combined with the \hc\ data increases the observational time baseline to $3238$\,days. Taking the ratio of these two time periods, the standard devation in period may be estimated at $0.019879$\,days or $28.62699$\,minutes.

\begin{figure}
    \centering
    \includegraphics[width=12cm]{Figures/V_period.pdf}
    \caption{\textbf{Top left:} Shown is a Lombscargle periodogram \citep{1982ApJ...263..835S} of V\,$1490$\,Cyg's light curve in the V filter. The period is determined to be $31.46700075$\,days for data with a magnitude uncertainty of less than $0.2$\,mag. \textbf{Top right:} The full V filter light curve of V\,$1490$\,Cyg. \textbf{Bottom:} The phase plot of V\,$1490$\,Cyg showing two full periods.}
    \label{fig:periodogram_V}
\end{figure}
        
\begin{figure}
    \centering
    \includegraphics[width=12cm]{Figures/R_period.pdf}
    \caption{\textbf{Top left:} Shown is a Lombscargle periodogram of V\,$1490$\,Cyg's light curve in the r filter. The period is determined to be $31.46694418$\,days for data with a magnitude uncertainty of less than $0.2$\,mag. \textbf{Top right:} The full r filter light curve of V\,$1490$\,Cyg. \textbf{Bottom:} The phase plot of V\,$1490$\,Cyg showing two full periods.}
    \label{fig:periodogram_R}
\end{figure}
        
\begin{figure}
    \centering
    \includegraphics[width=12cm]{Figures/I_period.pdf}
    \caption{\textbf{Top left:} Shown is a Lombscargle periodogram of V\,$1490$\,Cyg's light curve in the i filter. The period is determined to be $31.46703831$\,days for data with a magnitude uncertainty of less than $0.2$\,mag. \textbf{Top right:} The full i filter light curve of V\,$1490$\,Cyg. \textbf{Bottom:} The phase plot of V\,$1490$\,Cyg showing two full periods.}
    \label{fig:periodogram_I}
\end{figure}

Periodicity is also observed in the B-band data. However, due to fewer observations than Vri filters, the calculated period is given as $14.442371$\,days. Given further observations, this period is expected to begin to match that of Vri. The periodogram for the B-band data is shown in Fig.\,\ref{fig:periodogram_B}. Using just the \hc\ data, a period of $31.138910$\,days was found.

\begin{figure}
    \centering
    \includegraphics[width=12cm]{Figures/B_period.pdf}
    \caption{\textbf{Top left:} Shown is a Lombscargle periodogram of V\,$1490$\,Cyg's light curve in the B filter. The period is determined to be $14.44237126$\,days for data with a magnitude uncertainty of less than $0.2$\,mag. \textbf{Top right:} The full B filter light curve of V\,$1490$\,Cyg. \textbf{Bottom:} The phase plot of V\,$1490$\,Cyg showing two full periods.}
    \label{fig:periodogram_B}
\end{figure}

Light curves may also be asymmetric with respect to a reflection along the magnitude axis. Some stars show sharp increases in flux with others displaying prominent downward dips. It is believed that this behaviour is connected with the physical mechanisms causing variability. Upon visual inspection of V\,$1490$\,Cyg's light curve shown in Fig.\,\ref{fig:lightcurves}, one can see a clear dipping pattern in B, V, r and i filters. \citet{2014AJ....147...82C} developed an asymmetry metric $M$ to determine to what extent such asymmetry occurs. 

\begin{equation}
    \label{eq:Asymmetry_Metric}
    M = \frac{\left<d_{10\,\%}\right> - d_{\text{med}}}{\sigma_d}
\end{equation}

Following the method established in \citet{2014AJ....147...82C}, I determined $M$ for the V data of V\,$1490$\,Cyg, using Eqn.\,\ref{eq:Asymmetry_Metric}. $\left<d_{10\,\%}\right>$ is the mean of all magnitudes in the top and bottom ten percent of the V-Band light curve, $d_{med}$ the median of all V magnitudes and $\sigma_d$ the overall RMS of the V-Band data-points from the mean.

As detailed in \citet{2014AJ....147...82C}, objects with negative values are classified as bursters. These are objects that show short duration increases in brightness compared to their normal magnitudes. Conversely, objects with positive values for $M$ are dippers, which have short duration decreases in brightness compared to their normal state.

\citet{2014AJ....147...82C} use $\pm\,0.25$ as thresholds for $M$ to identify bursters and dippers. In the analysis of targets in \citet{2018MNRAS.478.5091F}, a slightly more conservative value was employed, identifying a burster as having $M < -0.5$, and a value of $M > 0.5$ considered a dipper. Objects with $M$ values in-between these borders are considered to have a symmetric behaviour. This threshold was raised to $M \pm 0.75$ for the most extreme bursters and dippers. The flux asymmetry ($M$) for the Visual light curve of V\,$1490$\,Cyg is calculated to be $0.819$. Following the criteria set above, this indicates that V\,$1490$\,Cyg may be classified as an  extreme dipper.

%----------------------------------------------------------------------------------------
%	Analysis of column density distribution of consecutive dips
%----------------------------------------------------------------------------------------
\subsection{Analysis of column density distribution of consecutive dips} 
\label{Analysis:column_density}

The quasi-periodic nature of \vc indicates orbital material held in place within a disk structure. As evidenced in the variability fingerprint plots described in Sect.\,\ref{Analysis:Fingerprint}, there is a significant probability that the source does not return to the exact same brightness after one full period. This indicates variation in the internal structure of the dips for each observation. Comparison of such flux variations in consecutive dips allows for an estimate to be made for the timescale on which the material is held in place.

V-band observations of \vc were folded in phase space with a period of $31.46699$\,days. The phase shift was calculated from the phase zero point when the object is bright. Figure\,\ref{fig:phased_V} shows the full phased V-band light curve of \vc. Indicated by the solid line is the running mean magnitude along with estimates of the running minimum (dashed line) and maximum (dash-dotted line) values. The deepest part of the dip occurs at a phase of roughly $0.6$. Magnitude scatter across phase space further supports inconsistency in the shape of consecutive dips indicating variation in internal structure. 

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/dip_change_analysis_1.pdf}
    \caption{Phased light curve of V-band data for \vc. Phase is determined with a period of $31.46699$\,days with a zero point of JD = $2458622.0$. The solid line indicated the running mean magnitude with the dashed and the dash-dotted lines showing the running minimum and maximum magnitudes respectively.}
    \label{fig:phased_V}
\end{figure}

If there were two clumps of orbiting material on opposite sides of the disk, the period observed would actually be half the correct period. To see if this is the case, consecutive dips and dips two periods apart were observed to compare their structure. Assuming differing yet stable properties for the two clump scenario, every second dip would show similar dimming trends.

For each observation in Fig.\,\ref{fig:phased_V}, a check was made to find all observations one period ahead, $\pm 1$\,day. If multiple matches were found, the magnitudes of matching observations were averaged by the mean of the magnitudes. The magnitude difference between this mean magnitude and that of the initial observation is plotted in phase space for all observations. The process is repeated but for a time gap of two periods $\pm 1$\,day. The left and right top two panels of Fig.\,\ref{fig:dip_change_analysis_2} show this magnitude difference between observations in phase space for one and two period separations respectively. The lower two panels show the absolute values seen in the top two panels.

The large scatter for both left and right panels indicates that the occulting material is different each time and that no obvious trend exists to suggest a two clump scenario.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/dip_change_analysis_2.pdf}
    \caption{\textbf{Top:} The two panels show the magnitude difference between observations in phase space and the mean magnitude of observations $1$\,period $\pm 1$\,day (left) and $2$\,periods $\pm 1$\,day (right) away. \textbf{Bottom:} The two panels show the absolute magnitude difference between observations in phase space and the mean magnitude of observations $1$\,period $\pm 1$\,day (left) and $2$\,periods $\pm 1$\,day (right) away.}
    \label{fig:dip_change_analysis_2}
\end{figure}

One is able to see how consecutive dips vary across the phase by averaging the phase plot into bins. Figure\,\ref{fig:dip_change_analysis_3} shows this for consecutive dips one period apart. Each phase bin is 10\,\% of the phase, inclusive of the upper limit. The left panel shows the mean and the right the median magnitude difference between dips.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/dip_change_analysis_3.pdf}
    \caption{\textbf{Left:} Mean magnitude difference for consecutive dips. Errorbars show mean rms scatter. \textbf{Right:} Median magnitude difference for consecutive dips. Errorbars show root median square scatter.}
    \label{fig:dip_change_analysis_3}
\end{figure}

Both panels agree on the shape of consecutive dips, with the median having a lower RMS scatter. This analysis may be run over consecutive dips n periods apart. Figure\,\ref{fig:dip_change_delta_1} displays the shape of consecutive dips for magnitude differences calculated for $1 - 10$ periods $\pm 1$\,day. By observing the range of flux variation, it may be noted that there is similar scatter over all values of n, though with differing shapes. For such an occurrence, the timescale of material held in the clump must be less than one period.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/dip_change_delta_1.pdf}
    \caption{\textbf{Left:} Mean magnitude difference across phase space for n - consecutive dips. \textbf{Right:} Median magnitude difference across phase space for n - consecutive dips.}
    \label{fig:dip_change_delta_1}
\end{figure}

To further analyse shape variations across n period separated dips, Fig.\,\ref{fig:dip_change_delta_2} displays the RMS magnitude scatter for bins in phase space. Bins are determined as for Fig.\,\ref{fig:dip_change_analysis_3}. For all observation matches within the bin, upper limit inclusive, RMS scatter was calculated and plotted, with the mean value shown in hatching.

The shape of each dip appears random across all values of n. This evidence further supports timescale of held material less than that of one full period. For material to build up across multiple periods before releasing onto the central object, lower n would show similar trends in their shape. Values of n greater than the timescale between which material is released would then become more random with increasing n. This behaviour is not observed in Fig.\,\ref{fig:dip_change_delta_2}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/dip_change_delta_2.pdf}
    \caption{Magnitude difference between consecutive dips in phase space. The bin size is 0.1, with upper limit inclusive. Mean Scatter is indicated in hatching.}
    \label{fig:dip_change_delta_2}
\end{figure}

The time of each observation in V-band data for \vc was converted into the number of periods away from a given start date. This date of JD = $2457237.45244$ was calculated by taking the earliest date of V-band data and subtracting the phase of that observation multiplied by the period of $31.46699$\,days.

For each observation, if the date mod $2$ yielded $0$, the observation was classified as being in an even period dip. If the date mod $2$ yielded $1$ then the observation was classified as being in an odd period dip. A check was made to find the magnitude difference between each observation and the median of observations $2$ periods $\pm 0.1$ phase away. The standard deviation was also determined. The median magnitude difference was then determined for all observations in integer periods such that a comparison is made between odd dips and even dips for increasing time.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/dip_change_1_period.pdf}
    \caption{Magnitude differences between consecutive dips two periods apart for V-band data of \vc. Shown in cross hatching are bars of even dips (time mod 1 = 0) and odd dips (time mod 1 = 1) are shown in diagonal hatching. Bars with no associated error contain only one data-point.}
    \label{fig:dip_change_1_period}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/dip_change_delta_3.pdf}
    \caption{Magnitude differences between consecutive dips two periods apart for V-band data of \vc. Shown in cross hatching are bars of even dips (time mod 2 = 0) and odd dips (time mod 2 = 1) are shown in diagonal hatching. Bars with no associated error contain only one data-point.}
    \label{fig:dip_change_delta_3}
\end{figure}

This analysis is shown in Fig.\,\ref{fig:dip_change_delta_3}, with even dips shown by light red bars with cross hatching and odd by light blue bars with diagonal hatching. Any bars with no error bars are comprised only of one matching observation.

One is able to see a random pattern of alternating dimming and brightening for both odd dip comparisons and even dips. This random nature of dip to dip events enhances the previous observations that the orbital material held in the disk is homogeneous showing no repeating structural patterns and moves though on a timescale less than the observed period.


%----------------------------------------------------------------------------------------
%	Analysis of the Variability Fingerprint Plots
%----------------------------------------------------------------------------------------


\subsection{Analysis of the Variability Fingerprint Plots}
\label{Analysis:Fingerprint}

Figure\,\ref{fig:fingerprints} shows the probability of flux variation over given timescales for UBVri\ha\ data of V\,$1490$\,Cyg. The bins are scaled in log base 10. Clearly recovered is the period of approximately $31.46699$\,days at a time-stamp of $\approx1.5$. BVri plots display very similar trends over all timescales with and U, \ha\ extremely variable on short timescales.

These variability fingerprint plots are created by calculating magnitude differences between observations in a given filter across all possible time gaps. A bicubic interpolation is used upon the resulting 2d histogram to smooth the bins and each bin column normalised. The colour bar range was limited to a 10\,\% maxima to show the detailed variation across the timescales.

U-band variability is seen to "increase" in brightness over times of $2.4$\,hours then fluctuating by $3.5$\,mag on timescales closer to $7 -- 8$\,hours. This aligns with what is observed of short-term U-band flux in the lower panel of Fig.\,\ref{fig:ds9_plots}. Long-term variation is not visible for U as there is limited data at this time.

Variability in \ha\ also shows abrupt changes in direction across small time-steps, though not to the same degree as in U. Variation is typically between $2$ and $2.5$\,mag on small timescales with some greater variability seen at around $100$\,days.

B, V, r and i plots all show some stability over short timescales but increase in variability toward larger timescales. In addition to the recovered period, one may see similar clumping at integer multiples of the period.

\begin{figure}
\centering
\makebox[\textwidth][c]{\includegraphics[width=0.7\textwidth]{images/U_fingerprint.pdf} \hfill \includegraphics[width=0.7\textwidth]{images/B_fingerprint.pdf} }\\%
\vspace{0.3cm}
\makebox[\textwidth][c]{\includegraphics[width=0.7\textwidth]{images/V_fingerprint.pdf} \hfill \includegraphics[width=0.7\textwidth]{images/R_fingerprint.pdf} }\\%
\vspace{0.3cm}
\makebox[\textwidth][c]{\includegraphics[width=0.7\textwidth]{images/I_fingerprint.pdf} \hfill \includegraphics[width=0.7\textwidth]{images/HA_fingerprint.pdf} }\\%
\caption{Variability fingerprint plots of U, B, V, r, i and \ha\ data for V\,$1490$\,Cyg are shown from left to right, top to bottom. The plots are normalised along the y-axis to give a probability of variability over a given timescale. Clearly observed in all BVri images is the periodicity of V\,$1490$\,Cyg, seen at $\approx1.5$ on the log time scale. This equates to a periodicity of roughly $31.46699$\,days as determined in Sect.\,\ref{Analysis:Periodic_Dipping_Behaviour}.}
\label{fig:fingerprints}
\end{figure}

%----------------------------------------------------------------------------------------
%	Analysis for the R-Ha and the Ha spectra from LCO
%----------------------------------------------------------------------------------------
\subsection{Analysis for the R-Ha and the Ha spectra from LCO}
\label{Analysis:Spectra}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/HA_lightcurve_zoom.pdf}
    \caption{The \ha-band light curve of V\,$1490$\,Cyg showing the dates of spectra.}
    \label{fig:HA_lightcurve}
\end{figure}

%----------------------------------------------------------------------------------------
%	Dust Scattering Properties
%----------------------------------------------------------------------------------------
\subsection{Dust scattering properties}
\label{Analysis:Dust_Scattering_Properties}

Analysis of the colour changes during dips, i.e. the slope in $V$ vs $V - i$ allows an insight into the dust scattering properties of the disk material. The value of this slope, the $\alpha$ parameter, indicates the amount of colour change during brightness change. Objects with large values (close to $90\,\degree$) virtually do not change their colour. Such objects could be eclipsing binaries with both components having similar colours. Any changes in flux caused by variability in the volume of absorbing and scattering material along the line of sight (e.g. from the accretion disk) typically changes the colour.

Using a standard reddening law \citep{1990ARA&A..28...37M}, disk material made from normal ISM dust would have $\alpha$-values between $60\,\degree$ ($R_V = 3.1$) and $66\,\degree$ ($R_V = 5.0$). Higher values of $\alpha$ less than $90\,\degree$ are possible if the obscuring material is made of larger dust grains than in the normal ISM or is optically thick.

Light curves with $\alpha < 55\,\degree$ are therefore not consistent with variability due to changes in extinction alone, but are most likely caused by changes in accretion rates or hot/cold surface spots. Objects that show $\alpha \approx 45\,\degree$ change their brightness in the V-band but not at a detectable level in the i-band. This can in principle be caused by non-variable red sources which are at the detection limit in V but detected at high signal-to-noise in the i-Band. Alternatively, these objects can be interpreted as sources with large fluctuations at visual wavelengths and small, undetected variations in the infrared. 

Many sources will have properties that indicate a mix of more than one of these physical reasons for variability. Hence, such categories bounding the $\alpha$-value are only suggestive of the main reason of variability for an object.

I calculate $\alpha$ for V\,$1490$\,Cyg by fitting a linear function (see Eq.\,\ref{eq:linear_alpha_func}) to the $N$ data-points in the $V - i$ vs. $V$ colour-magnitude diagram. This slope is indicated as a solid green line in Fig.\,\ref{fig:alpha_av}. The slope was determined by minimising the sum over all perpendicular distances of the data-points to the line of best fit (see Eq.\,\ref{eq:line_best_fit}). $\alpha$-values were converted into degrees to avoid the usage of large numerical values.

\begin{equation}
    V = V_0 + \alpha\left(V - i\right)
    \label{eq:linear_alpha_func}
\end{equation}

\begin{equation}
    \sum^N_{i=1}\frac{\left| V_0 \left(V - i\right) + \alpha - V \right|}{\sqrt{V_0^2 + 1}}
    \label{eq:line_best_fit}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/col_mag_plot.pdf}
    \caption{ Shown is the V vs V - i colour-magnitude diagram for V\,$1490$\,Cyg. The solid green line is a fit to the data, while the dash-dotted blue and dashed orange lines indicate $1$\,mag optical extinction vectors for $R_V = 3.1$ and $5.0$, respectively. The median $\alpha$-value of the V data is $74\,\degree$.}
    \label{fig:col_mag_plot}
\end{figure}

Plotting the $\alpha$-value against $A_v$ for all observations further than $5\sigma$ from the baseline ($15.4$\,mag), it may be seen there there is a linear trend, with a median $\alpha$-value of $(74\,\pm\,5)\,\degree$. The colour-magnitude variations of V\,$1490$\,Cyg are in agreement with variability caused by changes in the intervening column density of material composed of larger than normal ISM dust or opaque material. This is further indicated by the steep vector in the V vs V-I colour-magnitude diagram shown in Fig.\,\ref{fig:col_mag_plot}. There are no measurable changes in the dust scattering properties, neither with $A_V$ nor from dip to dip.

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/alpha_av.pdf}
    \caption{Black dots show the $\alpha$-value for each observation in the V data for V\,$1490$\,Cyg. Points were removed within $5\sigma$ of the baseline of $15.4$\,mag. Blue squared points are any with an $\alpha$-value $> 90\,\degree$. The red dashed line indicates the median $\alpha$-value of $(74\,\pm\,5)\,\degree$.}
    \label{fig:alpha_av}
\end{figure}

If the determination of the star's colour in Sect.\,\ref{Data:Colour_Correction} is incorrectly determined, a systematic offset is observed. Figure\,\ref{fig:alpha_av_shifted} shows all $\alpha$-values against $A_V$ when overestimating V\,$1490$\,Cyg's colour by $0.5$\,mag (V - i). It may be seen that the only effect of over-estimation is a systematic shift of $\alpha$-values upward with the median value raised by $2$\,\degree.

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/alpha_av_shifted.pdf}
    \caption{Black dots show the $\alpha$-value for each observation in the V data for V\,$1490$\,Cyg with the colour (V - i) overestimated by $0.5$\,mag. Points were removed within $5\sigma$ of the baseline of $15.4$\,mag. Blue squared points are any with an $\alpha$-value $> 90\,\degree$. The red dashed line indicates the median $\alpha$-value of $(76\,\pm\,5)\,\degree$}
    \label{fig:alpha_av_shifted}
\end{figure}

